Parameterized Analysis of Reconfigurable Broadcast Networks (Long Version)

Reconfigurable broadcast networks (RBN) are a model of distributed computation in which agents can broadcast messages to other agents using some underlying communication topology which can change arbitrarily over the course of executions. In this paper, we conduct parameterized analysis of RBN. We consider cubes,(infinite) sets of configurations in the form of lower and upper bounds on the number of agents in each state, and we show that we can evaluate boolean combinations over cubes and reachability sets of cubes in PSPACE. In particular, reachability from a cube to another cube is a PSPACE-complete problem. To prove the upper bound for this parameterized analysis, we prove some structural properties about the reachability sets and the symbolic graph abstraction of RBN, which might be of independent interest. We justify this claim by providing two applications of these results. First, we show that the almost-sure coverability problem is PSPACE-complete for RBN, thereby closing a complexity gap from a previous paper. Second, we define a computation model using RBN, \`a la population protocols, called RBN protocols. We characterize precisely the set of predicates that can be computed by such protocols.

==> poststar-cube.tex <==
%!TEX root = main.tex
\newcommand{\symbcube	}{\Delta_\cube}
\newcommand{\cubemin}{\cube_\gamma^\theta}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Counting sets are closed under reachability}

\chanain{I write the following sections assuming $\doublec{\theta}$ defined with $ \gamma(q) \ge v(q)$ instead of  $>$ on $S$}
In this subsection, we show that given a cube $\cube$, $\poststar(\cube)$ is  a counting set of bounded size. 
%We fix an arbitrary RBN $\RBN$ for the rest of the section.
We start by drawing links between cubes and symbolic configurations.
\begin{itemize}
\item Given a symbolic configuration $\theta=(v,S)$,
we define $\cube_\theta$ to be the cube $(L,U)$ 
such that $L=v$, and $U(q)=v(q)$ if $q \notin S$ and $U(q)=\infty$ otherwise.
Then $\cube_\theta = \doublec{\theta}$.
\item Given a cube $\cube=(L,U)$,
we define $\symbcube$ to be the set of symbolic configurations
$\theta=(v,S)$ with $S = \set{q | U(q)= \infty}$ and with $L(q) \le v(q) \le U(q)$ if $q \notin S$ and $v(q)=L(q)$ otherwise. 
Then $\doublec{\symbcube} = \cube$.
\end{itemize}
%\begin{definition}
%Let $\theta=(v,S)$ be a symbolic configuration. 
%We define $\cube_\theta$ to be the cube $(L,U)$ 
%such that $L=v$, and $U(q)=v(q)$ if $q \notin S$ and $U(q)=\infty$ otherwise.
%This set is such that $\cube_\theta = \doublec{\theta}$.
%
%Let $\cube=(L,U)$ be a cube.
%We define $\symbcube$ to be the set of symbolic configurations
%$\theta=(v,S)$ with $S = \set{q | U(q)= \infty}$ and with $L(q) \le v(q) \le U(q)$ if $q \notin S$ and $v(q)=L(q)$ otherwise. 
%This set is such that $\doublec{\symbcube} = \cube$.
%\end{definition}

Notice that $\symbcube$ is included in the symbolic graph of index $\norm{\cube}$.
\chana{well... I'm using the norm from our old io-rbn-sms draft, and it's $max(\sum L,\sum U)$, which can be smaller than $\sum_q max(L(q),U(q))$ ...maybe update norm or say we are in symb graph of index $2\norm{\cube}$ (update in pf thm2)}
By Remark \ref{rmk:symbgraph-reach}, 
we know that symbolic configurations in the graph of index $\norm{\cube}$ 
can only reach symbolic configurations also in  the graph of index $\norm{\cube}$,
of which there are a finite number.
Therefore $\poststar(\symbcube)$ is a finite set of symbolic configurations $\theta$.
It follows that $\doublec{\poststar(\symbcube)}$ is the finite union of the cubes $\cube_\theta$, and thus a counting set.

Unfortunately, it is in general not the case that $\poststar(\cube)= \doublec{\poststar(\symbcube)}$, which would close our argument.
However, we will show that for each symbolic configuration $\theta$ in $\poststar(\symbcube)$,
there is a counting set $\cSet_\theta \subseteq \doublec{\theta}$ 
such that the finite union of these counting sets is equal to $\poststar(\cube)$.
To define these counting sets, we first give ourselves an order on symbolic configurations and then prove a ``compatibility" lemma. \chana{the def and the lemma could be in the section above}

\begin{definition}
\label{def:symbconfig-order}
Let $\theta = (v,S)$ be a symbolic configuration, and let $\gamma, \gamma'$ be two configurations of $\RBN$.
We define an order $\preceq_{\theta}$ such that $\gamma \preceq_{\theta} \gamma'$ if and only if $\gamma ,\gamma' \in \doublec{ \theta}$, and $\forall q \in S$, $\gamma(q) \leq \gamma'(q)$.
\end{definition}

\begin{lemma}[Compatibility]
\label{lemma-poststar}
Let $\theta $ be a symbolic configuration, 
and let $\gamma, \gamma'$ be two configurations of $\RBN$.
If $\gamma \in \doublec{\theta}$ and $\gamma \act{*} \gamma'$,
then there exists a symbolic configuration $\theta'$ such that 
$\gamma' \in \doublec{\theta'}$ and $\theta \act{*}_\gr \theta'$ and for all configuration $\gamma'_1$ 
such  that $\gamma'_1 \succeq_{\theta'} \gamma'$,  there exists a configuration $\gamma_1 \in \doublec{\theta}$ such that $\gamma_1 \act{*} \gamma'_1$.
\end{lemma}
%
\begin{proof}
Let $\theta\in\Theta$ and $\gamma, \gamma', \gamma'_1 \in \Gamma$ such that $\gamma\in \doublec{\theta}$, and $\gamma\act{*}\gamma'$.
Let $\gamma = \gamma_0 \act{} \cdots\act{} \gamma_{m-1} \act{} \gamma_m = \gamma'$ denote the run between $\gamma$ and $\gamma'$.
We prove the property by induction on $m$. 
	For $m =0$, we have $\gamma= \gamma'$. The property  holds with $\theta' = \theta$, and $\gamma_1 = \gamma'_1$.
	
	Suppose now that $m \geq 1$, and that the property holds for all $n \leq m$. 
	By induction hypothesis, there exists $\theta_{m-1}$ satisfying the  property, in particular $\theta \act{*}_\gr \theta_{m-1}$.
	Since $\gamma_{m-1} \act{} \gamma_m$, by Lemma \ref{lm:runs},  
	there exists $\theta_m \in \Theta$ such that $\gamma_m \in \doublec{\theta_m}$, and $\theta_m = \theta_{m-1}$ or $\theta_{m-1} \act{}_\gr \theta_m$. Using $\theta \act{*}_\gr \theta_{m-1}$, we obtain that $\theta \act{*}_\gr \theta_m$.
	We note $\theta_{m-1} =(v_{m-1},S_{m-1})$ and $\theta_m = (v_m, S_m)$. 
	
	Let $\gamma'_m \in \doublec{\theta_m}$ be such that $\gamma'_m \succeq_{\theta_m} \gamma_m$. We want to build $\gamma'_{m-1}\in \doublec{\theta_{m-1}}$ such that $\gamma'_{m-1} \act{} \gamma'_m$.
Since we want $\gamma'_{m-1}\in \doublec{\theta_{m-1}}$, let $\gamma'_{m-1}(q) =   \gamma_{m-1}(q)$	for all $q \not \in S_{m-1}$.
To define $\gamma'_{m-1}$ on $S_{m-1}$, 
we define a  mapping $\emph{pred}$ from states in $S_m$ to states of $ S_{m-1} \cup  \overline{S_{m-1}}=Q$ as follows:
	\begin{itemize}
		\item if $q' \in S_{m-1}$, $\emph{pred}(q') = q'$;
		\item if $q' \not \in S_{m-1}$, by definition of transitions in the symbolic graph, there exists $q \in S_{m-1}$ such that $q \rightarrow^a q'$. Then $\emph{pred}(q') = q$ for one (arbitrary  but fixed) such $q$.
		\chana{check that there can indeed be more than one}
	\end{itemize} 
	By definition, $ \gamma'_m(q)= \gamma_m(q) $ for all $q \not \in S_m$. 
	For all $q \in S_m$, let $n_q =   \gamma'_m(q) -   \gamma_m(q)$. 
	Intuitively, we want to place these $n_q$ processes in the right places of $\gamma'_{m-1}$ so that $\gamma'_{m-1} \act{} \gamma'_m$. 	
	For all $q \in S_{m-1}$, let $  \gamma'_{m-1}(q) =   \gamma_{m-1}(q) + \sum_{q' \in S_m,\emph{pred}(q') = q} n_{q'}$. 
	By definition, $\gamma'_{m-1} \succeq \gamma_{m-1}$.
By the induction hypothesis, there exists $\gamma_1 \in \doublec{\theta}$ such that $\gamma_1\act{*} \gamma'_{m-1}$.
So all that remains is to prove  that $\gamma'_{m-1} \act{*} \gamma'_m$.
 
	We note $(p, !a, p')$ the broadcast rule between $\gamma_{m-1}$ and $\gamma_m$.
	From $\gamma'_{m-1}$, apply the broadcast rule $(p, !a, p')$. There are two cases. First, if $  \gamma'_{m-1}(p) =   \gamma_{m-1}(p)$, we consider the following transition in the RBN: all processes taking a reception transition between $\gamma_{m-1}$ and $\gamma_m$ do the same, and, in addition, for all $q$ such that $ \gamma'_{m-1}(q) >   \gamma_{m-1}(q)$, for all $q' \in S_m$ such that $\emph{pred}(q') = q$, $n_{q'}$ processes take the transition $(q, ?a, q')$. This way, we reach $\gamma'_m$. Now, if $  \gamma'_{m-1}(p) >   \gamma_{m-1}(p)$, we do the same to reach a configuration that we name $\gamma''$ such that $\forall q \in Q \setminus \{p, p'\}$, $  \gamma''(q) =   \gamma'_m(q)$ but $  \gamma''(p) =   \gamma'_m(p) + n_{p'}$ and $  \gamma''(p') =   \gamma'_m(p') - n_{p'} $. We can apply the broadcast rule $(p, !a ,p')$ $n_{p'}$ times with no  receives, and  reach $\gamma'_m$. Hence, $\gamma_1 \act{*} \gamma'_m$ which concludes the proof.
	\chana{beautify this last paragraph}
\end{proof}


\begin{theorem}
\label{thm:poststar}
Let $\cube$ be a cube of an RBN of state set $Q$. \chana{or should the bound be written out?}
Then $\poststar(\cube)$ is a counting set and
$$
\norm{\poststar(\cube)} \in O((\norm{\cube} \cdot |Q|)^{|Q|+2})
$$
The same holds for $\prestar$ by using the RBN with reversed transitions.
\end{theorem}
%
\begin{proof}
We start by defining a counting set $\mathcal{M}$ of configurations, 
which we will then prove to be equal to $\poststar(\cube)$.

Given a symbolic configuration $\theta$ of $\poststar(\symbcube)$,
we define the set $\min(\theta,\cube)$ of 
configurations $\gamma \in \doublec{\theta}$ such that $\gamma$ is minimal 
for the order $\preceq_{\theta}$ over the configurations of $\poststar(\cube)$, i.e.
$$
\min(\theta,\cube) = \min_{\preceq_{\theta}} \set{\gamma \in \doublec{\theta} | \gamma \in \poststar(\cube)}
$$
We can now define $\mathcal{M}$ to be the following set
$$
\mathcal{M}= \bigcup_{\theta \in \poststar(\symbcube)} \ \bigcup_{\gamma \in \min(\theta,\cube)} \cubemin,
$$
where $\cubemin$ is the cube $\cube_{(\gamma,S)}$ for $S$ such that $\theta=(v,S)$.
Since it is  a finite union of cubes, $\mathcal{M}$ is a counting set.

We show that $\poststar(\cube) \subseteq \mathcal{M}$.
Let $\gamma$ be a configuration in $\poststar(\cube)$.
There exists $\gamma_0 \in \cube$ such that $\gamma_0 \act{*} \gamma$, 
and there exists $\theta_0 \in \symbcube$ such that $\gamma_0 \in \doublec{\theta_0}$.
Applying Lemma \ref{lm:runs},
we obtain the existence of $\theta \in \poststar(\theta_0)\subseteq \poststar(\symbcube)$ such that $\gamma \in \doublec{\theta}$.
There exists a configuration $\gamma' \in \min(\theta,\cube)$ 
such that $\gamma' \preceq_{\theta}\gamma$.
Configuration $\gamma$ is in $\cube_{\gamma'}^\theta$ and thus in $\mathcal{M}$.

In the other direction, $\mathcal{M} \subseteq \poststar(\cube)$. 
Indeed each configuration $\gamma$ of $\mathcal{M}$ is in $\doublec{\theta}$
for a  $\theta \in \poststar(\symbcube)$, and 
there is a $\gamma' \in \poststar(\cube)$ such that $\gamma' \preceq_{\theta}\gamma$.
By Lemma \ref{lemma-poststar}, $\gamma$ is in $\poststar(\cube)$ as well.

Moreover, by Theorem \ref{theorem-upperboundN} and the fact that 
both $\symbcube$ and $\poststar(\symbcube)$ are in the graph of index $\norm{\cube}$, \chana{check coherence of index}
there exists an $N\le \norm{\cube} \times (2\norm{\cube})^{|Q|} \times (|Q|+1)^{|Q|+1}$ such that
for every $\gamma$ in $\doublec{\poststar(\symbcube)}_N$,
there exists a $\gamma_0 \in  \doublec{\symbcube}$ 
such that $\gamma_0 \act{*} \gamma$.
Since $\doublec{\symbcube}=\cube$, this  entails $\gamma \in \poststar(\cube)$.
That is, $\doublec{\poststar(\symbcube)}_N \subseteq \poststar(\cube)$.

Let $\theta = (v,S)$ be in $\poststar(\symbcube)$.
We can choose a $\gamma_N \in \doublec{\poststar(\symbcube)}_N$ that is also in $\doublec{\theta}$.
Then, since $\doublec{\poststar(\symbcube)}_N \subseteq \poststar(\cube)$
and by definition of $\min(\theta,\cube)$, 
 every $\gamma \in \min(\theta,\cube)$ is
such that $\gamma \preceq_\theta \gamma_N$. Thus
$\gamma(q) = v(q)$ if $q \notin S$ and $\gamma(q) \le v(q) + N$ otherwise. \chana{check coherence of $<$}
%Recall that a configuration $\gamma$ is in $\doublec{(v,S)}_N$ 
%if  $\gamma(q) = v(q)$ if $q \notin S$ and $\gamma(q) > v(q) + N$ otherwise.
Since $\theta = (v,S)$ is in $\poststar(\symbcube)$, $|v| \le \norm{\cube}$
and so $|\gamma| \le \norm{\cube} + |Q|N$.
The norm $\norm{\cubemin}$ is equal to $|\gamma|$.
Therefore $\norm{\cubemin}\le \norm{\cube} + |Q|N$.
Finally, using that the norm of a union of cubes is the maximum of the the cubes' norms, we obtain 
$$
\norm{ \poststar(\cube)} \le \norm{\cube} + |Q|N.
$$
By replacing $N$ by its upper bound we obtain our result. 

The results also hold for $\prestar(\cube)$. 
Consider the ``reverse" RBN net $\RBN_r$, defined as $\RBN=(Q,\Sigma,R)$ but with transition set $R_r$, where $R_r$ has a transition $(q, \star a, q')$ for $\star \in \set{!,?}$ 
if{}f $R_r$ has a transition $(q', \star a, q)$. 
Notice that $\RBN_r$ is still an RBN.
Then $\post^*(\cube)$ in $\RBN$ is equal to $\pre^*(\cube)$ in $\RBN_r$.
\end{proof}


Recall that counting sets are closed under boolean operations. With the above theorem, we obtain the following closure result.

\begin{corollary}[Closure]
\label{coro:closure}
Counting sets are closed under $\poststar$, $\prestar$ and boolean operations.
\end{corollary}


\begin{comment}

\begin{theorem}\label{theorem-poststar}
	Let $\varphi$ be a cube constraint. $\poststar{\varphi}$ is a finite union of cube constraints.
\end{theorem}

\begin{proof}
	We even show that we can describe $\poststar{\varphi}$ with at most $ |Q|! \times |Q|^{2\text{psize}(\varphi)} \times 2^{2|Q|}$ cubes. Let $\gamma' \in \poststar{\varphi}$, as $\poststar{\varphi} \subseteq \poststar{\mathcal{S}}$, there exists $\theta \in \mathcal{S}$, $\theta' = (v',S')$ such that $\theta \arrowstar{} \theta'$. From \ref{lemma-poststar}, there are at most $|S'|!$ minimal configurations $\gamma' \in \doublec{ \theta'}$. Indeed, otherwise we would have $\gamma \not = \gamma'$ such that $\gamma \succeq_{\theta'} \gamma'$ and $\gamma_0, \gamma'_0 \in \doublec{\theta}$, $\gamma_0 \act{*} \gamma$ and $\gamma'_0 \act{*} \gamma'$, which is absurd given that $\gamma$ and $\gamma'$ are minimals. Hence, we can enumerate the set of minimals configurations $M$, with $|M| \leq |Q|!$ and describe $\doublec{\theta'}$ as $\bigvee_{\gamma \in M} (\bigwedge_{q \in S'}   \gamma(q) \leq   q < \infty \wedge \bigwedge_{q \not \in S'}   q =   \gamma(q))$. As there are at most $|Q|^{\text{psize}(\varphi)} \times 2^{|Q|}$ such $\theta' \in \poststar{\mathcal{S}}$, and at most $|Q|^{\text{psize}(\varphi)} \times 2^{|Q|}$ such $\theta \in \mathcal{S}$, we get that to describe $\poststar{\varphi}$, we need a union of at most $ |Q|! \times |Q|^{2\text{psize}(\varphi)} \times 2^{2|Q|}$ constraint cubes.
\end{proof}

\begin{theorem}\label{theorem-psize-poststar}
	Let $\varphi$ be a cube constraint. $\text{psize}(\poststar{\varphi}) \leq \text{psize}(\varphi) + (|Q| + 1)^{|Q| + \text{psize}(\varphi)} \times 2^{|Q|}$.
\end{theorem}
\begin{proof}
	Immediately, if $Q = Q_0$, then $\poststar{\varphi} \subseteq \poststar{\theta_0}$.
	From \ref{theorem-upperboundN}, for all $\theta \in \poststar{\theta_0}$, $\exists N \leq (|Q| + 1)^{|Q| + \text{psize}(\varphi)} \times 2^{|Q|}$ such that for all $\gamma \in \doublec{\theta}_N$, we can reach it from an initial configuration. Hence, it goes the same for any $\theta =(v,S)$ such that $\doublec{\theta} \subseteq \poststar{\varphi}$. Hence, a minimal configuration of \ref{lemma-poststar} is smaller than the configuration $\gamma$ described by: for all $q \in S$, $  \gamma(q) = N +   v(q)$ and for all $q \not \in S$, $  \gamma(q) =   v(q)$. Therefore, each cubes of the union that we defined in the proof of \ref{theorem-poststar} can be described with natural numbers smaller than $\text{psize}(\varphi) + (|Q| + 1)^{|Q| + \text{psize}(\varphi)} \times 2^{|Q|}$. As a consequence, $\text{psize}(\poststar{\varphi}) \leq \text{psize}(\varphi) + (|Q| + 1)^{|Q| + \text{psize}(\varphi)} \times 2^{|Q|}$.
\end{proof}
\end{comment}

==> prop-symbolic-graph.tex <==
%!TEX root = main.tex
\subsection{Properties of the symbolic graph}

In this subsection, we prove some properties of the symbolic graph (of any index $k$). These properties will ultimately lead us to relate
paths over the symbolic graph to runs over the configurations of $\RBN$, which in turn will help us to prove our first main result in the 
next subsection.

Let $k \in \nn$ and let $\gr_k$ be the symbolic graph of index $k$ associated with $\RBN$. The first key property of $\gr_k$ is the following 
property, which we call \emph{monotonicity}. 

\begin{proposition}[Monotonicity]\label{prop-monotone}
	Let $\theta = (v,S)$ and $\theta' = (v', S')$. Then the following are true:
	\begin{itemize}
		\item If $Z \subseteq S$ and $\theta \act{a}_{\gr_k} \theta'$, then $(v, S) \act{a}_{\gr_k} (v', Z \cup S')$. 
		\item If $Z \subseteq Q$ and $\theta \act{a}_{\gr_k} \theta'$, then $(v, Z \cup S) \act{a}_{\gr_k} (v', Z \cup S')$.
	\end{itemize}	
\end{proposition}

\begin{proof}
	The two points follow in a straightforward manner from the definition of $\act{a}_{\gr_k}$.
	%For the third point, note that if $(v,S) \actsymb{} (v_1,S_1) \actsymb{} (v_2,S_2) \dots (v_{m-1},S_{m-1}) \actsymb{} (v',S')$ then
	%by the first two points, we have $(v,S) \actsymb{} (v_1, Z \cup S_1) \actsymb{} (v_2, Z \cup S_2) \dots (v_{m-1}, Z \cup S_{m-1}) \actsymb{} (v', Z \cup S')$.
\end{proof} 

To state the second property, we need a small definition first.
\begin{definition}
	Let $(v_0, S_0) \act{}_{\gr_k} \cdots \act{}_{\gr_k} (v_m, S_m)$ a path in the symbolic graph. 
	A pair of indices $0 \le i < j \le m$ is called a \emph{bad pair} if $(S_i \setminus S_{i+1}) \cap S_j \neq \emptyset$. 
	A path is said to be in \emph{normal form} if it contains no bad pairs, i.e., 
	for all $0 \le i < m$ and any $j > i$,
	$(S_i \setminus S_{i+1}) \cap S_j = \emptyset$. 
\end{definition}
Intuitively, a path is in normal form if during each step the set of states that disappear from the
abstract part never reappear again.  The following lemma asserts that whenever there is a path between two symbolic configurations,
then there is a path between them in normal form. 

\begin{lemma}[Normal Form]~\label{lemma-nf}
	Let $\theta, \theta' \in \Theta$ such that there is a path between $\theta$ and $\theta'$ of length $m$.
	Then, there is a path in normal form between $\theta$ and $\theta'$ of length $m$.
\end{lemma}

\begin{proof}
	Let $\theta = \theta_0 \actsymb{} \theta_1 \actsymb{} \theta_2 \actsymb{} \dots \theta_{m-1} \actsymb{} \theta_m = \theta'$ be the path between $\theta$ and $\theta'$.
	We proceed by induction on $m$. The claim is clearly true for $m = 0$. Suppose $m > 0$ and the claim is true for $m-1$. By induction hypothesis, we can assume 
	that the path $\theta_0 \actsymb{} \theta_1 \actsymb{} \dots \actsymb{} \theta_{m-1}$ is already in normal form.
	
	Let each $\theta_i = (v_i,S_i)$. Let $l$ be the number of bad pairs in the path between $\theta_0$ and $\theta_m$. If $l = 0$, then the path is already in normal form we are done.
	Suppose $l > 0$ and let $(w,w')$ be a bad pair. Since the path between $\theta_0$ and $\theta_{m-1}$ is already in normal form, it has to be the case that $w' = m$.
	Hence, we have $Z := (S_{w} \setminus S_{w+1}) \cap S_m \neq \emptyset$.
	
	By Proposition~\ref{prop-monotone}, the following is a valid path: $(v_{w},S_{w}) \actsymb{} (v_{w+1},S_{w+1} \cup Z) \actsymb{} (v_{w+2},S_{w+2} \cup Z) \dots (v_{m-1}, S_{m-1} \cup Z)\actsymb{} (v_m, S_m \cup Z) = (v_m,S_m)$. 
	Let $\theta'_j := \theta_j$ if $j \le w$ and $(v_j,S_j \cup Z)$ otherwise. 
	Hence, we get a path $\theta'_0 \actsymb{} \theta'_1 \actsymb{} \dots \theta'_{m-1} \actsymb{} \theta'_m$.
	
	Let each $\theta'_i = (v_i',S_i')$. We first claim that the path between $\theta'_0$ and $\theta'_{m-1}$ is in normal form. 
	Indeed, suppose there exists $0 \le i < j \le m-1$ such that $(S_i' \setminus S_{i+1}') \cap S_j' \neq \emptyset$. There are four cases:
	\begin{itemize}
		\item $i \le w$ and $j \le w$ : In this case $S_i' \setminus S_{i+1}' = S_i \setminus S_{i+1}$ and $S_j' = S_j$, and since the path between $\theta_0$ and $\theta_{m-1}$ is in normal form, this case cannot happen.
		\item $w < i$ and $w < j$: In this case $S_i' \setminus S_{i+1}' = S_i \setminus S_{i+1}$ and $S_j' = S_j \cup Z$. Since the path between $\theta_0$ and $\theta_{m-1}$ is in normal form, this should then 
		imply that $(S_i \setminus S_{i+1}) \cap Z \neq \emptyset$. By definition this means that $(S_w \setminus S_{w+1}) \cap S_i \neq \emptyset$ which contradicts the fact
		that the path between $\theta_0$ and $\theta_{m-1}$ is in normal form.
		\item $i < w$ and $w < j$: Similar to the case before, this should then imply that $(S_i \setminus S_{i+1}) \cap Z \neq \emptyset$. 
		By definition this means that $(S_i \setminus S_{i+1}) \cap S_w \neq \emptyset$ which contradicts the fact
		that the path between $\theta_0$ and $\theta_{m-1}$ is in normal form.
		\item $i = w$ and $w < j$: In this case $S_i' \setminus S_{i+1}' = S_i \setminus (S_{i+1} \cup Z)$ and $S_j' = S_j \cup Z$.  This
		would then imply that $(S_i \setminus S_{i+1}) \cap S_j \neq \emptyset$ which contradicts the fact
		that the path between $\theta_0$ and $\theta_{m-1}$ is in normal form.
	\end{itemize}
	
	It is then clear by construction, that this new path has $l-1$ bad pairs only.
	Hence, we now have a path from $\theta_0$ to $\theta_m$ such that the prefix of length $m-1$ is in normal form and the number of bad pairs has been strictly reduced to $l-1$.
	Repeatedly applying this procedure, leads to a path in normal form between $\theta_0$ and $\theta_m$.
\end{proof}

Before we state the third property, we need a small definition. Recall that given a symbolic configuration $\theta = (v,S)$, 
the set $\supp{\theta}$ denotes the set of configurations $\gamma$ such that $\gamma(q) = v(q)$ if $q \notin S$ and $\gamma(q) > v(q)$ otherwise.
The following definition refines the set $\supp{\theta}$.
\begin{definition}
	Given a symbolic configuration $\theta = (v,S)$ and a number $N \in \nn$, let $\supp{\theta}_N$ denote the set of configurations
	$\gamma$ such that $\gamma(q) = v(q)$ if $q \notin S$ and $\gamma(q) > v(q) + N$ otherwise. Note that $\supp{\theta} = \supp{\theta}_0$.
\end{definition}

This definition along with the above two properties now enable us to prove the following theorem, which relates paths over the symbolic graph to runs over the set of configurations.
It roughly states that if a symbolic configuration $\theta'$ can be reached from another symbolic configuration $\theta$ in the symbolic graph, then 
for a sufficiently large $N$, any configuration in $\supp{\theta'}_N$ can be reached from some configuration in $\supp{\theta}$.

\begin{theorem}\label{theorem-upperboundN}
	Let $\theta, \theta'$ be symbolic configurations of $\gr_k$ such that $\theta \actsymb{*} \theta'$.
	Then, there exists $N \leq k \times (2k)^{|Q|} \times (|Q|+1)^{|Q|+1}$ such that for all $\gamma' \in \supp{\theta'}_N$, there exists $\gamma \in \supp{\theta}$ such that $\gamma \act{*} \gamma'$.
\end{theorem}
 
\begin{proof}
	Suppose $\theta \actsymb{*} \theta'$. If the length of the path is 0, then there is nothing to prove.
	Hence, we restrict ourselves to the case when the length of the path is bigger than 0.
	By Lemma~\ref{lemma-nf}, there is a path in normal from from $\theta$ to $\theta'$ (say)
	$\theta = \theta_0 \actsymb{} \theta_1 \actsymb{} \theta_2 \dots \theta_{m-1} \actsymb{} \theta_m = \theta'$ with each
	$\theta_i := (v_i,S_i)$. 
	
	Let $N_0 = 0$ and let $N_i = (N_{i-1}+1) \cdot (|S_{i-1} \setminus S_i|+1)$ for every $1 \le i \le m$. 
	In Lemma 6 of~\cite{Delzanno12}, the following fact has been proved: 
	\begin{quote}
		For every $1 \le i \le m$ and for every $\gamma' \in \supp{\theta_i}_{N_i}$, there exists $\gamma \in \supp{\theta_{i-1}}_{N_{i-1}}$ such that
		$\gamma \act{*} \gamma'$.
	\end{quote}
	
	This immediately proves that for all $\gamma' \in \supp{\theta'}_{N_m}$, there exists $\gamma \in \supp{\theta}$ such that $\gamma \act{*} \gamma'$. If we prove $N_m \le k \times (2k)^{|Q|} \times (|Q|+1)^{|Q|+1}$, then the proof of the theorem will be complete.

	Notice that since the path between $\theta_0$ and $\theta_m$ is in normal form, the number of indices $i$ such that $|S_{i-1} \setminus S_i| > 0$
	is at most $|Q|$. Indeed, suppose $q \in S_{i-1} \setminus S_i$ for some $i$. Then by the normal form property, $q \notin S_j$ for any $j \ge i$. 
	Hence, in the rest of the path $q$ does not appear in the abstract part at all. By definition of the edges in the symbolic graph, 
	there can be no outgoing edges from a symbolic configuration whose abstract part is the empty set. These two facts then imply that
	the number of indices $i$ such that $|S_{i-1} \setminus S_i| > 0$
	is at most $|Q|$.
	
	It then follows that except for at most $|Q|$ indices, each index $N_i$ is obtained from $N_{i-1}$ by simply adding 1
	and in the remaining indices, $N_i$ is obtained from $N_{i-1}$ by adding 1 and then multiplying by a number which is at most $|Q|+1$.
	The way to maximize $N_m$ by this procedure is by letting $N_i = N_{i-1} + 1$ for every $1 \le i \le m-|Q|$ and then
	letting $N_i = (N_{i-1}+1) \cdot (|Q|+1)$ for every $m-|Q| < i \le m$. This gives an upper bound 
	of $(m-|Q|+1)|Q|(|Q|+1)^{|Q|}$ for $N_m$. Since $m$ is itself the length of the path between $\theta_0$ and $\theta_m$,
	$m$ is upper bounded by the number of symbolic configurations in $\gr_k$ which is at most $|\nn_k^{Q}| \times 2^{|Q|} \le k \times k^{|Q|} \times 2^{|Q|}$.
	Overall we get that $N_m \le k \times (2k)^{|Q|} \times (|Q|+1)^{|Q|+1}$.
\end{proof}


==> pspace-lemma.tex <==
%!TEX root = main.tex
\subsection{PSPACE Lemma/Everything is PSPACE (find better name)}

In this subsection, we use Theorem \ref{thm:poststar} to show our main result. 
We show that there exist \PSPACE{} algorithms to evaluate predicates with boolean and reachability operators over counting sets. \chana{say something abt writing counting sets/configs in binary}
This allows many parameterized problems for RBN to be solved in \PSPACE.
\chana{say that similar to DC, both énoncé and proof}

\begin{theorem}[Name]
\label{thm:pspace-lemma}
        Let $\mathcal{S}_1$ and $\mathcal{S}_2$ be two functions 
        that take as arguments a RBN $\RBN$ and a counting set $X$, and return counting sets $\mathcal{S}_1(\RBN,X)$ and $\mathcal{S}_2(\RBN,X)$ respectively.
  Assume that $\mathcal{S}_1(\RBN,X)$  and $\mathcal{S}_2(\RBN,X)$ 
        have
        norms at most exponential in the size of the $(\RBN,X)$,
        as well as
        \PSPACE{}-decidable membership
        (given input $(C,\RBN,X)$, decide whether $C \in \mathcal{S}_i(\RBN,X)$).
        
        Then the same is true about the counting sets
        $\mathcal{S}_1(\RBN,X)\cap\mathcal{S}_2(\RBN,X)$,
        $\mathcal{S}_1(\RBN,X)\cup\mathcal{S}_2(\RBN,X)$,
        $\compl{\mathcal{S}_1(\RBN,X)}$, and
        $\prestar(\mathcal{S}_1(\RBN,X))$.
        Furthermore, given $\RBN$ and $X$, the emptiness problem for these sets is in \PSPACE.
\end{theorem}
%
\begin{proof}%\chana{careful this is very like DC)}
        The exponential bounds for the norms follow immediately from 
        Proposition~\ref{prop:oponconf} and Theorem~\ref{thm:poststar}.
        The membership complexity for union, intersection and 
        complement is easy to see.
        Without loss of generality it suffices to prove that membership in
        $\poststar(\mathcal{S}_1(\net,X))$
        is in \PSPACE.

        By Savitch's Theorem \NPSPACE=\PSPACE, so we provide a nondeterministic algorithm.
        Given $(C,\net,X)$, we want to decide whether $C\in \poststar(\mathcal{S}_1(\net,X))$.
        The algorithm
        first guesses a configuration $C_0 \in \mathcal{S}_1(\net,X)$ of the same size as $C$,
        verifies that $C_0$ belongs to $\mathcal{S}_1(\net,X)$, 
        and then guesses an execution starting at $C_0$, step by step,
        checking after each step if the reached configuration is $C$.
        Notice that all intermediate configurations of such an execution have the same size as $C$.
        At any moment in time the algorithm only stores three configurations,
        the current one, the next configuration in the execution, and the input one. 
        %This concludes the proof of the claim.

        We can now observe that the  emptiness problem is in \PSPACE{} for any counting set
        with exponentially bounded norm and \PSPACE-decidable membership.
        We again use Savitch's Theorem.
        If the counting set is nonempty, it has an element
        of size smaller or equal to the norm of the set. \chana{explicit why?}
        Such an element can be described in polynomial space.
        Therefore we can guess it and verify the set membership.
\end{proof}

This result is a powerful tool which can be used to prove that a host of problems are in \PSPACE \ for RBN.
For example, checking whether there exists a configuration in $\cSet_1$ which can reach a configuration in $\cSet_2$
is equivalent to checking emptiness of $\poststar(\cSet_1) \cap \cSet_2$.
If we replace $\cSet_2$'s upper bounds with $\infty$ in the expression, checking emptiness is equivalent to checking whether $\cSet_2$ is coverable from $\cSet_1$.
Combining this with the fact that the reachability problem between two configurations of an RBN net is \PSPACE-hard, as shown in \cite{}\chana{cite RBN paper}, we obtain the following result.

\begin{theorem}
Cube-to-cube reachability and cube-to-cube coverability are \PSPACE-complete for RBN.
\end{theorem}

More complex problems can be expressed, 
for example in the context of stochastic schedulers. 
This is developped in the next section.

